Inertial manifolds and foliations for asymptotically compact cocycles in Banach spaces

We study asymptotically compact nonautonomous dynamical systems given by abstract cocycles in Banach spaces. Our main assumptions are given by a squeezing property in a quadratic cone field (given by a family of indefinite quadratic Lyapunov-like functionals) and asymptotic compactness. Under such conditions it is possible to reconstruct foliations as in the theory of normally hyperbolic manifolds. Our approach allows to unify many "practical" theories of local and nonlocal invariant manifolds, such as stable/unstable/center manifolds and inertial manifolds, and, moreover, it often leads to optimal conditions for their existence. We give applications for semilinear parabolic equations and neutral delay equations, where the Frequency Theorem is used to construct constant cone fields.

==> Differentiability.tex <==
\subsection{Differentiability (for semiflows)}
\label{SUBSEC: Differentiability}

Throughout this subsection we suppose that we are given with a semiflow $\varphi^{t} \colon \mathbb{E} \to \mathbb{E}$, where $t \geq 0$, which satisfies all the hypotheses of Theorem \ref{TH: InertialManifoldsExponentialTracking}, that is \textbf{(H1)},\textbf{(H2)}, \textbf{(H3)}, \textbf{(ULIP)}, \textbf{(COM)}. We will also assume that there is at least one amenable trajectory. Note that \textbf{(PROJ)} is automatically satisfied since there is no dependence on $q$ of all the operators and spaces in \textbf{(H1)}. So, \textbf{(H1)} means that there exists an operator $P \in \mathcal{L}(\mathbb{E})$ and a decomposition $\mathbb{E} = \mathbb{E}^{+} \oplus \mathbb{E}^{-}$ such that $P$ is positive on $\mathbb{E}^{+}$ and negative on $\mathbb{E}^{-}$; \textbf{(H2)} means that $\operatorname{dim}\mathbb{E}^{-} = j$; \textbf{(H3)} means that the inequality
\begin{equation}
	\label{EQ: H3Semiflow}
	e^{2\nu r}V(\varphi^{r}(v_{1})-\varphi^{r}(v_{2})) - V(v_{1}-v_{2}) \leq -\delta \int_{0}^{r}e^{2\nu s} |\varphi^{s}(v_{1})-\varphi^{s}(v_{2})|^{2}_{\mathbb{H}}ds.
\end{equation}
is satisfied for all $r \geq \tau_{V}$ and all $v_{1},v_{2} \in \mathbb{E}$. Here $V(v):=\langle v , Pv \rangle$ is the quadratic form of $P$. We recall that $\nu > 0$, $\tau_{V} \geq 0$ and $\delta > 0$ are some constants.

Let $\Pi \colon \mathbb{E} \to \mathbb{E}^{-}$ be the $V$-orthogonal projector (see Remark \ref{REM: Orthogonality}). By Theorem \ref{TH: InertialManifolds} there is a $j$-dimensional topological manifold $\mathfrak{A}$ and $\Pi \colon \mathfrak{A} \to \mathbb{E}^{-}$ is a homeomorphism. Let $\Phi \colon \mathbb{E}^{-} \to \mathfrak{A}$ be the inverse to $\Pi \colon \mathfrak{A} \to \mathbb{E}^{-}$. From Lemma \ref{LEM: PhiLipschitz} it follows that $\Phi$ is Lipschitz and, consequently, $\mathfrak{A}$ is a Lipschitz submanifold in $\mathbb{E}$. Here we will study differentiability properties of $\mathfrak{A}$.

Since for every $t \geq 0$ the map $\varphi^{t}$ is bijective on $\mathfrak{A}$, its inverse is continuous by the Brouwer theorem on invariance of domain and, consequently, the restriction of $\varphi$ to $\mathfrak{A}$ is a flow. We will assume that there exists a linearization of $\varphi$ on $\mathfrak{A}$, which is a linear cocycle, as follows.
\begin{description}
	\item[$\text{\textbf{(DIFF)}}_{\varphi}$] There exists a linear cocycle $\psi$ in $\mathbb{E}$ over the flow $(\mathfrak{A},\varphi)$, which satisfies \textbf{(ULIP)} and \textbf{(COM)}, and such that for all $v \in \mathfrak{A}$ and $\xi \in \mathbb{E}$ the limit
	\begin{equation}
		\label{EQ: LinearizationCocycleLimit}
		\lim_{h \to 0+} \frac{ \varphi^{t}(v + h\xi) - \varphi^{t}(v)}{h} = \psi^{t}(v,\xi)
	\end{equation}
    exists in $\mathbb{H}$ for all $t \geq 0$. Moreover, for a fixed $t \geq \tau_{V}$ the limit in \eqref{EQ: LinearizationCocycleLimit} exists in $\mathbb{E}$ and is uniform in $\xi$ from compact subsets of $\mathbb{E}$. 
\end{description}
We refer to $\psi$ as the \textit{linearization cocycle}. To emphasize that the map $\psi^{t}(v,\cdot)$ is linear we usually write $L(t;v)\xi$ instead of $\psi^{t}(v,\xi)$. The linear map $L(t;v)$ is called the \textit{quasi-differential} of $\varphi^{t}$ at $v$. In applications, $\psi$ is obtained through some linearized differential equation.

The first observation is that the linearization cocycle of a semi-flow, which satisfies \textbf{(H1)},\textbf{(H2)} and \textbf{(H3)}, also satisfies these properties w.~r.~t. the same constant operator $P$ and the constant decomposition $\mathbb{E}=\mathbb{E}^{+} \oplus \mathbb{E}^{-}$. This is contained in the following lemma.
\begin{lemma}
	 Let $\text{\textbf{(DIFF)}}_{\varphi}$ be satisfied. Then we have
	 \begin{equation}
	 	\label{EQ: H3LinCocycle}
	 	e^{2\nu r}V(L(r;v)\xi) - V(\xi) \leq -\delta \int_{0}^{r} e^{2 \nu s}|L(s;v)\xi|^{2}_{\mathbb{H}} ds
	 \end{equation}
     for all $r \geq \tau_{V}$, $\xi \in \mathbb{E}$ and $v \in \mathfrak{A}$.
\end{lemma}
\begin{proof}
	For are given $v \in \mathfrak{A}$ and $\xi \in \mathbb{E}$ we consider \eqref{EQ: H3Semiflow} with $v_{1} := v + h\xi$ and $v_{2} := v$ and divide both sides by $h^{2}$. Then, as $h \to 0$, the left-hand side of \eqref{EQ: H3Semiflow} tends to the left-hand side of \eqref{EQ: H3LinCocycle} (thanks to $\text{\textbf{(DIFF)}}_{\varphi}$) and the right-hand side of \eqref{EQ: H3Semiflow} tends to the right-hand side of \eqref{EQ: H3LinCocycle} by the dominated convergence theorem, which assumptions are satisfied because of $\text{\textbf{(DIFF)}}_{\varphi}$ and \textbf{(ULIP)} for the semiflow. Thus, \eqref{EQ: H3LinCocycle} is satisfied.
\end{proof}

Thus the linearization cocycle $\psi$ satisfies all the hypotheses of Theorem \ref{TH: InertialManifolds}. Note that for $v \in \mathfrak{A}$ there is always a zero compete trajectory, which is amenable. So, there is a family of $j$-dimensional linear subspaces $\mathfrak{A}(v)$, which forms the inertial manifold for the linearized cocycle given by Theorem \ref{TH: InertialManifolds}. Also there is a map $\Phi_{L} \colon \mathfrak{A} \times \mathbb{E}^{-} \to \mathbb{E}$ such that $\Phi_{L}(v,\eta) \in \mathfrak{A}(v)$ and $\Pi \Phi_{L}(v,\eta) = \eta$ for all $v \in \mathfrak{A}$ and $\eta \in \mathbb{E}^{-}$. Since $\Phi_{L}(v,\cdot)$ is linear, we usually write $\Phi_{L}(v)\eta$ instead of $\Phi_{L}(v,\eta)$. Our aim is to show that $\mathfrak{A}(v)$ is the tangent space of $\mathfrak{A}$ at $v$ and that $\Phi_{L}(v)$ is the differential of $\Phi$, which continuously depend on $v \in \mathfrak{A}$. The main theorem of this section is the following.
\begin{theorem}
	\label{TH: Differentiability}
	Let the semiflow satisfy $\text{\textbf{(DIFF)}}_{\varphi}$ and also $\text{\textbf{(DIFF)}}_{\Phi}$ and \textbf{(CDLIN)} defined below. Then $\mathfrak{A}$ is a $C^{1}$-differentiable submanifold in $\mathbb{E}$ and the flow $\varphi$ on $\mathfrak{A}$ is $C^{1}$-differentiable. Moreover, the tangent space at $v$ is given by $\mathfrak{A}(v)$ and $\Phi \colon \mathbb{E}^{-} \to \mathbb{E}$ is continuously Fr\'{e}chet differentiable such that $\Phi'(\zeta) = \Phi_{L}(\Phi(\zeta))$ for all $\zeta \in \mathbb{E}^{-}$.
\end{theorem}
It is known that $C^{1}$-differentiability of $\mathfrak{A}$ is the maximum that one can obtain using the classical Spectral Gap Condition (which is included in our theory as we will see in Subsection \ref{SUBSEC: SemilinearParabolicEquations}) for semilinear parabolic equations \cite{ChowLuSell1992}. To obtain some smoothness of higher order one needs a more restrictive condition \cite{ChowLuSell1992,RosaTemam1996}. The present author does not know how to describe these additional assumptions in terms of strengthened versions of \textbf{(H3)}.

It is clear that in order to prove Theorem \ref{TH: Differentiability} it is sufficient to establish its last statement. The proof below follows the ideas from our previous work \cite{Anikushin2020Semigroups}. Let us formulate an auxiliary lemma on the differentiability of Lipschitz mappings from \cite{Anikushin2020Semigroups}.
\begin{lemma}
	\label{LEM: AuxiliaryLemmaDiffLipMap}
	Let $F \colon \mathbb{R}^{m} \to \mathbb{H}_{aux}$ be a locally Lipschitz function with values in some Hilbert space $\mathbb{H}_{aux}$. Suppose also that $\mathbb{H}_{aux}$ is continuously embedded into $\mathbb{E}$. Let there exist a family of linear maps $D(x) \in \mathcal{L}(\mathbb{R}^{j};\mathbb{E})$, which continuously depend on $x \in \mathbb{R}^{m}$. Let $F'(x)=D(x)$ be satisfied for almost all $x \in \mathbb{R}^{m}$. Then $F \colon \mathbb{R}^{m} \to \mathbb{E}$ is continuously Fr\'{e}chet differentiable and $F'(x)=D(x)$ for all $x \in \mathbb{R}^{m}$.
\end{lemma}
\begin{proof}
	Let us start with the case $j=1$. The Lipschitz continuity implies that $F$ is absolutely continuous and, consequently, for all $x \in \mathbb{R}$ we have
	\begin{equation}
		F(x) - F(0) = \int_{0}^{x} F'(y) dy = \int_{0}^{x}D(y)dy.
	\end{equation}
	Since the function on the right-hand side is continuously differentiable with its derivative $D(x)$, the same holds for $F(\cdot)$.
	
	Now let us consider, for simplicity of notation, the case $j=2$ (the case $j>2$ can be treated analogously). Let $\mathcal{D}$ denote the unit disk and $\mathcal{S}^{1}$ denote the unit circle in $\mathbb{R}^{2}$. Our aim is to show that for all $x \in \mathbb{R}^{2}$ there is a dense subset of $\xi \in (\mathcal{S}^{1} + x)$ for which we have $F(x+t \xi) - F(x) = tD(x)\xi + o(t)$ as $t \to 0+$, where $t \in [0,1]$. Without loss of generality, we may assume that $x=0$. Let $\widetilde{D}$ denote the set of all $y \in \mathcal{D}$ for which we have $F'(y)=D(y)$. By assumption, $\lambda_{2}(\widetilde{D}) = \lambda_{2}(\mathcal{D}) = \pi$, where $\lambda_{2}(\cdot)$ denotes the two-dimensional Lebesgue measure. Consider the partition of $\mathcal{D}$ onto closed unit segments $\mathcal{I}_{\alpha}$ by the angle $\alpha \in [0,2\pi]$, i.~e. $\mathcal{I}_{0} := \{ (x_{1},0) \in \mathbb{R}^{2} \ | \ x_{1} \in [0,1] \}$ and $\mathcal{I}_{\alpha}$ is given by the rotation of $\mathcal{I}_{0}$ by $\alpha$. From the Fubini theorem we have
	\begin{equation}
		\label{EQ: LipLemma1Fubini}
		\pi = \lambda_{2}(\widetilde{\mathcal{D}}) = \frac{1}{2} \int_{0}^{2\pi} \lambda_{1}(\mathcal{I}_{\alpha} \cap \widetilde{\mathcal{D}}) d \alpha,
	\end{equation}
	where $\lambda_{1}$ denotes the one-dimensional Lebesgue measure. Consider the set $\mathcal{C}_{k}$ of all $\alpha \in [0,2\pi]$ such that $\lambda_{1}(\mathcal{I}_{\alpha} \cap \widetilde{\mathcal{D}}) \geq 1 - 1/k$. From \eqref{EQ: LipLemma1Fubini} it immediately follows that $\mathcal{C}_{k}$ is a set of full measure in $[0,2\pi]$. Then the set $\bigcap_{k=1}^{\infty}\mathcal{C}_{k}$ is also a set of full measure in $[0,2\pi]$. In particular, there is a dense set of $\alpha \in [0,2\pi]$, for which $F'(y)$ exists and $F'(y)=D(y)$ for almost all $y \in \mathcal{I}_{\alpha}$. Let $\xi_{\alpha} \in \mathcal{I}_{\alpha}$ be the unique unit vector, i.~e. $\mathcal{I}_{\alpha} = \bigcup_{t \in [0,1]} \{ t \xi_{\alpha} \}$. Then for such $\alpha$ the derivative of the Lipschitz function $F_{\alpha}(t) = F(t \xi_{\alpha})$ exists and coincides with $D(t\xi_{\alpha})\xi$ for almost all $t \in [0,1]$. From the previous case ($j=1$) we have that $F_{\alpha}$ is differentiable at $t = 0$ and $F(t \xi_{\alpha}) - F(0) = tD(0)\xi_{\alpha} + o(t)$.
	
	Now we will prove that $F(h)-F(0) = D(0)h + o(h)$ as $h \to 0$. Let $\varepsilon>0$ be fixed. Our aim is to find $\delta>0$ such that for some $C>0$ (independent of $\delta$)
	\begin{equation}
		\|(F(0+h)-F(0) - D(0)h) \|_{\mathbb{E}} \leq C\varepsilon |h|
	\end{equation}
	provided that $|h| < \delta$. Let $\xi_{l}$, where $l=1,2,\ldots,L$ for some $L>0$ be an $\varepsilon$-net on $\mathcal{S}^{1}$ such that $F(t \xi_{l}) - F(0) = tD(0)\xi_{l} + o(t)$ as $t \to 0$ for any $l$. Then we can find $\delta>0$ such that if $|t| < \delta$ then
	\begin{equation}
		\|F(t \xi_{l}) - F(0) - tD(0)\xi_{l}\|_{\mathbb{E}} < \varepsilon |t|.
	\end{equation}
	for all $l$. For any $h \in \mathbb{R}^{2}$ we put $\xi := \frac{h}{|h|}$. Then $h = |h| \xi$, where $\xi \in \mathcal{S}^{1}$. Let $1 \leq l_{0} \leq L$ be such that $|\xi_{l_{0}}-\xi| < \varepsilon$. Since $F$ is Lipschitz and $D(0)$ is bounded, there exists a constant $C>0$ such that
	\begin{equation}
		\begin{split}
			\|(F(h)-F(0) - D(0)h) \|_{\mathbb{E}} \leq \| F(h) - F(|h|\xi_{l_{0}}) \|_{\mathbb{E}} +\\+ \| F(|h|\xi_{l_{0}}) - F(0) - |h|D(0) \xi_{l_{0}} \|_{\mathbb{E}} + \| D(0)(|h|\xi_{l_{0}} - h) \|_{\mathbb{E}} \leq C \varepsilon |h|
		\end{split}
	\end{equation}
	provided that $|h| < \delta$. This gives the desired differentiability at $x=0$. Thus, $F'(x) = D(x)$ for all $x \in \mathbb{R}^{2}$ and the lemma is proved.
\end{proof}

We have to consider the following assumptions.
\begin{description}
	\item[$\textbf{(DIFF)}_{\Phi}$] There exists a Hilbert space $\mathbb{H}_{aux}$, which is continuously embedded into $\mathbb{E}$ and we have $\mathfrak{A} \subset \mathbb{H}_{aux}$ under the embedding. Moreover, the function $\Phi \colon \mathbb{E}^{-} \to \mathbb{H}_{aux}$ is locally Lipschitz.
\end{description}

Under $\textbf{(DIFF)}_{\Phi}$, from the Rademacher theorem we get that the function $\Phi \colon \mathbb{E}^{-} \to \mathbb{H}_{aux}$ has the the Fr\'{e}chet derivative $\Phi'(\zeta) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{H}_{aux})$ for almost all $\zeta \in \mathbb{E}^{-}$.

\begin{description}
	\item[\textbf{(CDLIN)}] The function $\Phi_{L} \colon \mathfrak{A} \times \mathbb{E}^{-} \to \mathbb{E}$ is continuous.
\end{description}
By Lemma \ref{LEM: PhiLipschitz}, the map $\Phi \colon \mathbb{E}^{-} \to \mathbb{E}$ is globally Lipschitz. Thus, if $\mathbb{E}$ is a Hilbert space, then $\textbf{(DIFF)}_{\Phi}$ is satisfied with $\mathbb{H}_{aux}$. In the general case the space $\mathbb{E}$ may not satisfy the Radon-Nikodym property and thus there may exist $\mathbb{E}$-valued Lipschitz mappings which are not differentiable almost everywhere. However, in such situations we usually have that $\Phi$ takes values in a some Hilbert space $\mathbb{H}_{aux}$ and $\textbf{(DIFF)}_{\Phi}$ is satisfied. See \cite{Anikushin2020Semigroups} for this.

To satisfy \textbf{(CDLIN)} it is sufficient for the cocycle to be uniformly compact in the sense of \textbf{(UCOM)} (see Lemma \ref{LEM: CocycleUniformCompactnessContinuity}) and in applications this property is a consequence of \textbf{(ULIP)} and some smoothing properties of differential equations.

Let $\mathcal{C}_{V}$ denote the set of all $v \in \mathbb{E}$ such that $V(v) \leq 0$. By the construction of $\mathfrak{A}$ and $\mathfrak{A}(v)$ we have $\mathfrak{A} \subset \mathcal{C}_{V}$ and $\mathfrak{A}(v) \subset \mathcal{C}_{V}$ for all $v \in \mathfrak{A}$ (see Lemma \ref{LEM: AmenableTrajectories}). The set $\mathcal{C}_{V}$ is a closed $j$-dimensional quadratic cone in $\mathbb{E}$ in the sense that $\mathcal{C}_{V}$ is closed, $\alpha v \in \mathcal{C}_{V}$ for any $\alpha \in \mathbb{R}$ and $v \in \mathcal{C}_{V}$ and $j$ is the maximal dimension of a linear subspace, which entirely lies in $\mathcal{C}_{V}$.

\begin{lemma}
	\label{LEM: DelayPhiDerivative1}
	Let $\text{\textbf{(DIFF)}}_{\varphi}$ be satisfied. Suppose that for some $\zeta_{0} \in \mathbb{E}^{-}$ there exists the Fr\'{e}chet derivative $\Phi'(\zeta_{0}) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$. Then we have
	\begin{enumerate}
		\item[1.] $\operatorname{dim} \Phi'(\zeta_{0}) \mathbb{E}^{-} = j$ and $\Phi'(\zeta_{0})\mathbb{E}^{-} \subset \mathcal{C}_{V}$. Moreover, $h = \Pi \Phi'(\zeta_{0}) h$ for all $h \in \mathbb{E}^{-}$.
		\item[2.] If $\Phi'(\zeta_{0})\mathbb{E}^{-} \subset \mathfrak{A}(\Phi(\zeta_{0}))$ then $\Phi'(\zeta_{0}) = \Phi_{L}(\Phi(\zeta_{0}))$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	1. By assumptions, we have 
	\begin{equation}
		\label{EQ: LemmaPhiDerBaseGen}
		\Phi(\zeta_{0} + h) - \Phi(\zeta_{0}) = \Phi'(\zeta_{0}) h + o(h)
	\end{equation}
	for all $h \in \mathbb{E}^{-}$. Taking $\Pi$ on both sides of \eqref{EQ: LemmaPhiDerBaseGen}, we get $h = \Pi \Phi'(\zeta_{0})h + o(h)$ or, since all the maps are linear and bounded, we get $h = \Pi \Phi'(\zeta_{0})h$ for all $h \in \mathbb{E}^{-}$. Thus, $\Phi'(\zeta_{0})$ is injective. Now for a fixed  $\zeta \in \mathbb{E}^{-}$ put $h = t \zeta$, where $t > 0$, in \eqref{EQ: LemmaPhiDerBaseGen} to get as $t \to 0$
	\begin{equation}
		\label{EQ: LemmaPhiDerCone}
		\frac{\Phi(\zeta_{0}+t\zeta)-\Phi(\zeta_{0})}{t} = \Phi'(\zeta_{0})\zeta + o(1).
	\end{equation}
	Note that the left-hand side of \eqref{EQ: LemmaPhiDerCone} lies in the cone $\mathcal{C}_{V}$. Taking it to the limit as $t \to 0$, we get that $\Phi'(\zeta_{0})\zeta \in \mathcal{C}_{V}$.
	
	2. Since $h = \Pi \Phi'(\zeta_{0})h$ for all $h \in \mathbb{E}^{-}$, we get that $\Pi$ is the left inverse of $\Phi'(\zeta_{0})$ on the image $\Phi'(\zeta_{0})\mathbb{E}^{-}$. If $\Phi'(\zeta_{0})\mathbb{E}^{-} \subset \mathfrak{A}(\Phi(\zeta_{0}))$, then it immediately follows from item 1 that $\Phi'(\zeta_{0})\mathbb{E}^{-} = \mathfrak{A}(\Phi(\zeta_{0}))$ and since, by definition, $\Pi$ is also the left-inverse for $\Phi_{L}(\Phi(\zeta_{0}))$ on $\mathfrak{A}(\Phi(\zeta_{0}))$, we get the identity $\Phi'(\zeta_{0}) = \Phi_{L}(\Phi(\zeta_{0}))$.
\end{proof}

For convenience sake, let us put $\mathbb{E}_{\zeta} := \Phi'(\zeta)\mathbb{E}^{-}$ if the Fr\'{e}chet derivative $\Phi'(\zeta) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$ is well-defined. Although our goal is to show that $\mathbb{E}_{\zeta} = \mathfrak{A}(\Phi(\zeta))$, we do not know this at the present moment. Let $\zeta(t;\zeta_{0})=\zeta^{t}(\zeta_{0}):=\Pi\varphi^{t}(\Phi(\zeta_{0}))$ be the flow $\varphi$ on $\mathfrak{A}$ projected to $\mathbb{E}^{-}$.

\begin{lemma}
	\label{LEM: DelayPhiDerivative2}
	Let $\text{\textbf{(DIFF)}}_{\varphi}$ be satisfied. Suppose that for some $\zeta_{0} \in \mathbb{E}^{-}$ there exists the Fr\'{e}chet derivative $\Phi'(\zeta_{0}) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$. Then for all $t \geq \tau_{V}$ there also exists the Fr\'{e}chet derivative $\Phi'(\zeta(t,\zeta_{0})) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$ and $L(t;\Phi(\zeta_{0})) \colon \mathbb{E}_{\zeta_{0}} \to \mathbb{E}_{\zeta(t;\zeta_{0})}$ is an isomorphism.
\end{lemma}
\begin{proof}
	Firstly, we will show that $L(t;\Phi(\zeta_{0}))$ is injective on $\mathbb{E}_{\zeta_{0}}$ for $t \geq 0$. Let $t \geq \tau_{V}$ be fixed. For $\xi \in \mathbb{E}_{\zeta_{0}}$ from \eqref{EQ: H3LinCocycle} we have
	\begin{equation}
		\label{EQ: LemPhiDer2H3}
		-e^{2\nu t}V(L(t,\Phi(\zeta_{0}))\xi) + V(\xi) \geq \delta \int_{0}^{t}e^{2\nu s}|L(s;\Phi(\zeta_{0}))\xi|^{2}_{\mathbb{H}}ds.
	\end{equation}
	By item 1 of Lemma \ref{LEM: DelayPhiDerivative1} we have $V(\xi) \leq 0$ and, consequently, $V(L(t,\Phi(\zeta_{0}))\xi) \leq 0$. Since the projector $\Pi$ is $V$-orthogonal, we have $-V(L(t,\Phi(\zeta_{0}))\xi) \leq \|P\| \cdot \|\Pi L(t;\Phi(\zeta_{0}))\xi\|^{2}_{\mathbb{E}}$. From this and \eqref{EQ: LemPhiDer2H3} we get
	\begin{equation}
		\label{EQ: LemPhiDer2H3Est}
		\delta^{-1} e^{2\nu t} \|P\| \cdot \| \Pi L(t;\Phi(\zeta_{0})) \xi \|^{2}_{\mathbb{E}} \geq \int_{0}^{t}e^{2\nu s} |L(s;\Phi(\zeta_{0}))\xi|^{2}_{\mathbb{H}} ds
	\end{equation}
	that immediately shows that $L(t;\Phi(\zeta_{0}))$ is injective for $t \geq \tau_{V}$. In virtue of the cocycle property for $L$, we have that $L(t;\Phi(\zeta_{0}))$ is injective for all $t \geq 0$. Put $\mathbb{E}^{(t)} := L(t;\Phi(\zeta_{0}))\mathbb{E}_{\zeta_{0}}$ that is a $j$-dimensional subspace of $\mathbb{E}$. From \eqref{EQ: LemPhiDer2H3Est} it is also follows that $\Pi$ is injective on $\mathbb{E}^{(t)}$. Let $\Pi_{t}$ denote the restriction of $\Pi$ to $\mathbb{E}^{(t)}$. Our aim is to show that $\Phi'(\zeta(t;\zeta_{0}))$ is given by the inverse of $\Pi_{t}$ for $t \geq \tau_{V}$.
	
	From $\text{\textbf{(DIFF)}}_{\varphi}$ for a fixed $t \geq \tau_{V}$ and $\widetilde{h} \in \mathbb{E}^{-}$ we get that
	\begin{equation}
		\label{EQ: LemPhiDer2Differentiability}
		\varphi^{t}(\Phi(\zeta_{0}+\widetilde{h})) - \varphi^{t}(\Phi(\zeta_{0})) = L(t;\Phi(\zeta_{0})\Phi'(\zeta_{0})\widetilde{h} + o(\widetilde{h}),
	\end{equation}
	where the smallness of $o(\widetilde{h})$ should be understanded in the norm of $\mathbb{E}$. Put 
	\begin{equation}
		\label{EQ: LemPhiDer2Hchoice}
		h := \Pi_{t} L(t;\Phi(\zeta_{0})) \Phi'(\zeta_{0}) \widetilde{h}.
	\end{equation}
	Then from \eqref{EQ: LemPhiDer2Differentiability}, \eqref{EQ: LemPhiDer2Hchoice} and the Lipschitz property of $\Phi$ we have
	\begin{equation}
		\begin{split}
			\Phi(\zeta(t;\zeta_{0})+h)-\Phi(\zeta(t;\zeta_{0})) = \\ = \Phi(\Pi\varphi^{t}(\Phi(\zeta_{0})) + h) - \Phi(\Pi \varphi^{t} (\Phi(\zeta_{0})) ) = \\ = \Phi(\Pi \varphi^{t}(\Phi(\zeta_{0} + \widetilde{h}) + o(\widetilde{h})) - \Phi(\Pi \varphi^{t}(\Phi(\zeta_{0}))) = \\ = \varphi^{t}(\Phi(\zeta_{0}+\widetilde{h})) - \varphi^{t}(\Phi(\zeta_{0})) + o(\widetilde{h}) =\\=  L(t;\Phi(\zeta_{0}))\Phi'(\zeta_{0}) \left[\Pi_{t} L(t;\Phi(\zeta_{0})) \Phi'(\zeta_{0})\right]^{-1} h + o(h) = \\ = \Pi_{t}^{-1} h + o (h).
		\end{split}	
	\end{equation}
	Thus, there exists the Fr\'{e}chet derivative $\Phi'(\zeta(t,\zeta_{0})) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$ and equals to $\Pi_{t}^{-1}$ for all $t \geq \tau_{V}$. The lemma is proved.
\end{proof}

The following lemma gives a criterion to determine the identity $\Phi'(\zeta_{0}) = \Phi_{L}(\Phi(\zeta_{0}))$ and it highly relies on the ideas from the proof of Theorem \ref{TH: InertialManifolds}. This is our final ingredient.

\begin{lemma}
	\label{LEM: DerCoincidenceCriteria}
	Let $\text{\textbf{(DIFF)}}_{\varphi}$ be satisfied. Suppose that for some $\zeta_{0} \in \mathbb{E}^{-}$ and a sequence $t_{k} \to -\infty$ there exists the Fr\'{e}chet derivative $\Phi'(\zeta(t_{k};\zeta_{0})) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$ for all $k=1,2,\ldots$. Then there also exists the Fr\'{e}chet derivative $\Phi'(\zeta_{0}) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$ and $\Phi'(\zeta_{0}) = \Phi_{L}(\Phi(\zeta_{0}))$.
\end{lemma}
\begin{proof}
	At first note that $\Phi'(\zeta_{0})$ exists thanks to Lemma \ref{LEM: DelayPhiDerivative2}. Let $\zeta \in \mathbb{E}$ be fixed. Our aim is to show that $\Phi'(\zeta_{0}) \zeta \in \mathfrak{A}(\Phi(\zeta_{0}))$. For this we will construct an amenable trajectory $\xi^{*}(\cdot)$ of the linearization cocycle passing through $\Phi'(\zeta_{0})\zeta$ at $\Phi(\zeta_{0})$ and such that $\Pi \xi(0) = \zeta$. Let us for every $k=1,2,\ldots$ define the trajectory $\xi_{k}(t)$ for $t \geq t_{k}$ as
	\begin{equation}
		\xi_{k}(t):=L(t-t_{k};\varphi^{t_{k}}(\Phi(\zeta_{0}))) \xi_{k,0},
	\end{equation}
	where $\xi_{k,0} \in \mathbb{E}_{\zeta(t_{k};\zeta_{0})}$ is chosen in such a way that $\Pi \xi_{k} = \zeta$. Such $\xi_{k,0}$ exists and unique due to Lemma \ref{LEM: DelayPhiDerivative2}. Note that $V(\xi_{k}(t)) \leq 0$ for all $t \geq t_{k}$. We have the estimate
	\begin{equation}
		\delta^{-1} \| P \| \cdot \| \zeta \|^{2}_{\mathbb{E}} \geq \int_{t_{k}}^{0}e^{2\nu s} |\xi_{k}(s)|^{2}_{\mathbb{H}}ds.
	\end{equation}
	From this we can obtain a subsequence (in the same way as in the proof of Lemma \ref{LEM: ManifoldConstruction}) of $\xi_{k}(\cdot)$ (we keep the same index) such that $\xi_{k}(t)$ converges in $\mathbb{E}$ to some complete trajectory $\xi^{*}(t)$ at $\Phi(\zeta_{0})$ uniformly in $t$ from compact intervals. It is clear that $V(\xi^{*}(t)) \leq 0$ for all $t \in \mathbb{R}$ and, by Lemma \ref{LEM: AmenableTrajectories}, $\xi^{*}(\cdot)$ is amenable. Since $\Pi \xi_{k}(0) = \zeta$, we have $\Pi \xi(0) = \zeta$. Moreover, $\xi(0) \in \mathbb{E}_{\zeta_{0}}$ since $\xi_{k}(0) \in \mathbb{E}_{\zeta_{0}}$. Therefore, by item 1 of Lemma \ref{LEM: DelayPhiDerivative1} we must have $\xi(0)=\Phi'(\zeta_{0})\zeta$ and, consequently, $\Phi'(\zeta_{0})\zeta \in \mathfrak{A}(\Phi(\zeta_{0}))$. Now item 2 of Lemma \ref{LEM: DelayPhiDerivative1} gives us the identity $\Phi'(\zeta_{0}) = \Phi_{L}(\Phi(\zeta_{0}))$.
\end{proof}

Now we can give a proof of Theorem \ref{TH: Differentiability}
\begin{proof}[Proof of Theorem \ref{TH: Differentiability}]
	It is easy to see that for almost all $\zeta_{0} \in \mathbb{E}^{-}$ for the sequence $t_{k} = -k$ we have the conditions of Lemma \ref{LEM: DerCoincidenceCriteria} satisfied. Indeed, $\Phi'(\zeta_{0}) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$ exists for all $\zeta_{0} \in \mathcal{B}$, where $\mathcal{B}$ is a set of full Lebesgue measure. For $k=1,2,\ldots $ consider the sets $\mathcal{B}_{k}:=\zeta^{k}(\mathcal{B})$, where $\zeta^{t}(\cdot)=\zeta(t;\cdot)$ is the projected flow. Clearly, for all $\zeta_{0} \in \mathcal{B}_{k}$ there exists the Fr\'{e}chet derivative $\Phi'(\zeta(-k;\zeta_{0})) \in \mathcal{L}(\mathbb{E}^{-};\mathbb{E})$. Since the map $\zeta_{0} \mapsto \zeta(t;\zeta_{0})$ is a Lipschitz homeomorphism of $\mathbb{E}^{-}$ (thanks to the Lipschitzity of $\Phi$ and $\Pi$ and \textbf{(ULIP)} property of $\varphi$), $\mathcal{B}_{k}$ is a set of full measure. Therefore, the intersection $\bigcap_{k=1}^{\infty}\mathcal{B}_{k}$ is also a set of full measure.
	
	Thus, \textbf{(CDLIN)} and Lemma \ref{LEM: DerCoincidenceCriteria} gives us the equality $\Phi'(\zeta_{0})=\Phi_{L}(\Phi(\zeta_{0}))$ for almost all $\zeta_{0} \in \mathbb{E}^{-}$. From Lemma \ref{LEM: AuxiliaryLemmaDiffLipMap} we have that $\Phi \colon \mathbb{E}^{-} \to \mathbb{E}$ is continuously differentiable with $\Phi'(\zeta_{0}) = \Phi_{L}(\Phi(\zeta_{0}))$ for all $\zeta_{0} \in \mathbb{E}^{-}$. From this it immediately follows that $\mathfrak{A}$ is a smooth submanifold in $\mathbb{E}$ and the tangent space at $v \in \mathfrak{A}$ is given by $\mathfrak{A}(v)$. To see that the flow $\varphi$ on $\mathfrak{A}$ is $C^{1}$-differentiable we use $\text{\textbf{(DIFF)}}_{\varphi}$ to get for a fixed $t \geq 0$ that
	\begin{equation}
		\varphi^{t}(\Phi(\zeta_{0} + h))-\varphi^{t}(\Phi(\zeta_{0})) = L(t;\Phi(\zeta_{0}))\Phi'(\zeta_{0}) + o(h).
	\end{equation}
    Taking $\Pi$ from both sides, we get
    \begin{equation}
    	\zeta^{t}(\zeta_{0}+h)-\zeta^{t}(\zeta_{0}) = \Pi L(t;\Phi(\zeta_{0}))\Phi'(\zeta_{0})h + o(h)
    \end{equation}
    that shows the required differentiability. Thus, the theorem is proved.
\end{proof}
